Modeling the Second Player in Distributionally Robust Optimization

Distributionally robust optimization (DRO) provides a framework for training machine learning models that are able to perform well on a collection of related data distributions (the "uncertainty set"). This is done by solving a min-max game: the model is trained to minimize its maximum expected loss among all distributions in the uncertainty set. While careful design of the uncertainty set is critical to the success of the DRO procedure, previous work has been limited to relatively simple alternatives that keep the min-max optimization problem exactly tractable, such as $f$-divergence balls. In this paper, we argue instead for the use of neural generative models to characterize the worst-case distribution, allowing for more flexible and problem-specific selection of the uncertainty set. However, while simple conceptually, this approach poses a number of implementation and optimization challenges. To circumvent these issues, we propose a relaxation of the KL-constrained inner maximization objective that makes the DRO problem more amenable to gradient-based optimization of large scale generative models, and develop model selection heuristics to guide hyper-parameter search. On both toy settings and realistic NLP tasks, we find that the proposed approach yields models that are more robust than comparable baselines.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/biased_sst_95_ablation.tex <==
% \begin{table}[t]
% \small
% \begin{center}
% \begin{tabular}{lccc}
% \toprule 
% Stopping strategy  & Average & Robust & Adversarial \\
% \midrule
% ERM & { 3.82} {\scriptsize$\pm$ 1.07} & { 18.60} {\scriptsize$\pm$ 2.83} & { 4.43} {\scriptsize$\pm$ 1.97} \\
% \cmidrule{2-4}
% $\lambda=10^{-4}$, $k=5$, $\tau=0.01$ & \underline{ 28.82} {\scriptsize$\pm$ 14.84} & \underline{ 43.58} {\scriptsize$\pm$ 5.14} & \underline{ 34.07} {\scriptsize$\pm$ 13.05} \\
% \cmidrule{2-4}
% $k=0$ & \underline{ 34.17} {\scriptsize$\pm$ 6.21} & \underline{ 36.66} {\scriptsize$\pm$ 5.41} & \underline{ 32.58} {\scriptsize$\pm$ 4.56} \\
% $k=10$ & \underline{ 33.17} {\scriptsize$\pm$ 16.92} & \underline{ 47.27} {\scriptsize$\pm$ 3.70} & \underline{ 43.54} {\scriptsize$\pm$ 2.16} \\
% \cmidrule{2-4}
% $\tau=0.1$ & { 20.14} {\scriptsize$\pm$ 12.41} & { 18.78} {\scriptsize$\pm$ 13.68} & \underline{ 20.53} {\scriptsize$\pm$ 10.60} \\
% $\tau=0.001$ & \underline{ 34.32} {\scriptsize$\pm$ 17.22} & \underline{ 40.53} {\scriptsize$\pm$ 9.42} & \underline{ 37.24} {\scriptsize$\pm$ 8.90} \\
% \cmidrule{2-4}
% $\lambda=10^{-3}$ & \underline{ 18.29} {\scriptsize$\pm$ 2.40} & \underline{ 20.56} {\scriptsize$\pm$ 8.26} & \underline{ 14.98} {\scriptsize$\pm$ 4.20} \\
% $\lambda=10^{-5}$ & { 14.49} {\scriptsize$\pm$ 21.51} & \underline{ 49.17} {\scriptsize$\pm$ 4.10} & { 22.30} {\scriptsize$\pm$ 22.91} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{\label{tab:hyperparams} Hyperparameter Change Effects ($\text{biased-SST}_{95}$). }
% \end{table}

\begin{table}[t]
\small
\begin{center}
\begin{tabular}{lccc}
\toprule 
\backslashbox{Configuration}{Stopping}   & Robust & Average & Adv Greedy\\
\midrule
ERM & { 23.64} {\scriptsize$\pm$ 3.40} & { 4.47} {\scriptsize$\pm$ 3.98} & { 4.47} {\scriptsize$\pm$ 3.98} \\
$\lambda=10^{-4}$, $k=5$, $\tau=0.01$ & \underline{ 46.96} {\scriptsize$\pm$ 6.73} & \underline{ 28.74} {\scriptsize$\pm$ 15.65} & \underline{ 33.08} {\scriptsize$\pm$ 11.70} \\
$\lambda=10^{-3}$ & { 28.38} {\scriptsize$\pm$ 4.87} & \underline{ 20.32} {\scriptsize$\pm$ 3.36} & \underline{ 21.23} {\scriptsize$\pm$ 4.36} \\
$\lambda=10^{-5}$ & \underline{ 53.68} {\scriptsize$\pm$ 8.14} & { 9.92} {\scriptsize$\pm$ 15.62} & { 18.62} {\scriptsize$\pm$ 19.33} \\
$\tau=0.1$ & { 25.22} {\scriptsize$\pm$ 13.86} & \underline{ 22.17} {\scriptsize$\pm$ 13.02} & { 22.77} {\scriptsize$\pm$ 15.75} \\
$\tau=0.001$ & \underline{ 45.61} {\scriptsize$\pm$ 5.83} & \underline{ 31.38} {\scriptsize$\pm$ 17.99} & \underline{ 31.62} {\scriptsize$\pm$ 12.01} \\
$k=0$ & { 35.65} {\scriptsize$\pm$ 7.73} & \underline{ 28.93} {\scriptsize$\pm$ 8.15} & \underline{ 27.71} {\scriptsize$\pm$ 10.45} \\
$k=10$ & \underline{ 47.35} {\scriptsize$\pm$ 4.81} & \underline{ 30.71} {\scriptsize$\pm$ 16.04} & \underline{ 37.94} {\scriptsize$\pm$ 5.98} \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:biased_sst_95_ablations_bilstm} Effect of Adv-DRO hyper-parameters on validation robust accuracy for the BiLSTM model ($\text{biased-SST}_{95}$). }
\end{table}



% \begin{table}[t]
% \small
% \begin{center}
% \begin{tabular}{lccccccc}
% \toprule 
% Stopping strategy  & Robust & Average & Warmup & Adv Nash & Adv Greedy & Nash (thresh) & Greedy (thresh) \\
% \midrule
% ERM & { 39.53} {\scriptsize$\pm$ 3.89} & { 11.16} {\scriptsize$\pm$ 10.02} & { 2.75} {\scriptsize$\pm$ 3.70} & { 11.16} {\scriptsize$\pm$ 10.02} & { 11.16} {\scriptsize$\pm$ 10.02} & { 11.16} {\scriptsize$\pm$ 10.02} & { 11.16} {\scriptsize$\pm$ 10.02} \\
% $k=0$ & { 43.32} {\scriptsize$\pm$ 9.11} & \underline{ 41.77} {\scriptsize$\pm$ 9.87} & \underline{ 38.05} {\scriptsize$\pm$ 9.23} & \underline{ 29.53} {\scriptsize$\pm$ 12.71} & \underline{ 29.53} {\scriptsize$\pm$ 12.71} & \underline{ 29.53} {\scriptsize$\pm$ 12.71} & \underline{ 29.53} {\scriptsize$\pm$ 12.71} \\
%  & { 47.03} {\scriptsize$\pm$ 5.75} & \underline{ 33.02} {\scriptsize$\pm$ 17.11} & \underline{ 41.63} {\scriptsize$\pm$ 9.92} & \underline{ 44.19} {\scriptsize$\pm$ 6.58} & \underline{ 44.19} {\scriptsize$\pm$ 6.58} & \underline{ 44.19} {\scriptsize$\pm$ 6.58} & \underline{ 44.19} {\scriptsize$\pm$ 6.58} \\
% $\tau=0.1$ & { 31.74} {\scriptsize$\pm$ 13.90} & { 27.65} {\scriptsize$\pm$ 16.28} & { 25.40} {\scriptsize$\pm$ 16.99} & { 27.16} {\scriptsize$\pm$ 16.36} & { 27.16} {\scriptsize$\pm$ 16.36} & { 27.16} {\scriptsize$\pm$ 16.36} & { 27.16} {\scriptsize$\pm$ 16.36} \\
% $\tau=0.001$ & \underline{ 48.88} {\scriptsize$\pm$ 4.86} & \underline{ 33.18} {\scriptsize$\pm$ 17.30} & \underline{ 45.61} {\scriptsize$\pm$ 6.18} & \underline{ 45.70} {\scriptsize$\pm$ 7.17} & \underline{ 45.70} {\scriptsize$\pm$ 7.17} & \underline{ 45.70} {\scriptsize$\pm$ 7.17} & \underline{ 45.70} {\scriptsize$\pm$ 7.17} \\
% $\lambda=10^{-3}$ & { 30.26} {\scriptsize$\pm$ 8.81} & { 21.21} {\scriptsize$\pm$ 7.72} & \underline{ 17.81} {\scriptsize$\pm$ 9.28} & { 14.29} {\scriptsize$\pm$ 6.32} & { 14.29} {\scriptsize$\pm$ 6.32} & { 16.92} {\scriptsize$\pm$ 5.99} & { 17.36} {\scriptsize$\pm$ 5.61} \\
% $\lambda=10^{-5}$ & \underline{ 56.03} {\scriptsize$\pm$ 2.56} & { 6.67} {\scriptsize$\pm$ 6.59} & { 16.01} {\scriptsize$\pm$ 18.74} & { 16.89} {\scriptsize$\pm$ 18.03} & { 16.89} {\scriptsize$\pm$ 18.03} & { 16.89} {\scriptsize$\pm$ 18.03} & { 16.89} {\scriptsize$\pm$ 18.03} \\
% $k=10$ & \underline{ 48.86} {\scriptsize$\pm$ 6.17} & \underline{ 32.65} {\scriptsize$\pm$ 16.94} & \underline{ 44.76} {\scriptsize$\pm$ 6.35} & \underline{ 44.24} {\scriptsize$\pm$ 7.92} & \underline{ 44.24} {\scriptsize$\pm$ 7.92} & \underline{ 44.24} {\scriptsize$\pm$ 7.92} & \underline{ 44.24} {\scriptsize$\pm$ 7.92} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{\label{tab:hyperparams} Hyperparameter Change Effects ($\text{biased-SST}_{90}$). }
% \end{table}



\begin{table}[t]
\small
\begin{center}
\begin{tabular}{lccc}
\toprule 
\backslashbox{Configuration}{Stopping}  & Robust & Average  & Adv Greedy  \\
\midrule
ERM & { 67.31} {\scriptsize$\pm$ 4.03} & { 57.27} {\scriptsize$\pm$ 4.64} & { 57.27} {\scriptsize$\pm$ 4.64} \\
$\lambda=10^{-4}$, $k=5$, $\tau=0.01$ & \underline{ 77.27} {\scriptsize$\pm$ 2.87} & \underline{ 66.09} {\scriptsize$\pm$ 4.45} & \underline{ 70.32} {\scriptsize$\pm$ 4.23} \\
$\lambda=10^{-3}$ & { 68.62} {\scriptsize$\pm$ 7.90} & { 51.82} {\scriptsize$\pm$ 8.91} & { 63.79} {\scriptsize$\pm$ 11.39} \\
$\lambda=10^{-5}$ & \underline{ 73.83} {\scriptsize$\pm$ 3.63} & \underline{ 66.36} {\scriptsize$\pm$ 4.61} & \underline{ 69.68} {\scriptsize$\pm$ 2.85} \\
$\tau=0.1$ & \underline{ 80.40} {\scriptsize$\pm$ 3.36} & { 65.73} {\scriptsize$\pm$ 2.60} & \underline{ 72.96} {\scriptsize$\pm$ 7.62} \\
$\tau=0.001$ & \underline{ 79.68} {\scriptsize$\pm$ 3.26} & \underline{ 65.22} {\scriptsize$\pm$ 2.79} & \underline{ 75.93} {\scriptsize$\pm$ 6.42} \\
$k=0$ & \underline{ 75.06} {\scriptsize$\pm$ 5.83} & { 62.85} {\scriptsize$\pm$ 4.25} & { 68.18} {\scriptsize$\pm$ 9.37} \\
$k=10$ & \underline{ 80.36} {\scriptsize$\pm$ 2.16} & \underline{ 70.75} {\scriptsize$\pm$ 2.63} & \underline{ 76.05} {\scriptsize$\pm$ 6.93} \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:biased_sst_95_ablations_bert} Effect of Adv-DRO hyper-parameters on validation robust accuracy for BERT ($\text{biased-SST}_{95}$), BERT. }
\end{table}

==> tables/biased_sst_95_model_selection.tex <==
\begin{table}[h]
% \small
\begin{center}
\begin{tabular}{llc}
\toprule
 Selection  & Robust accuracy \\
\midrule
% ERM & Average & { 2.05} {\scriptsize$\pm$ 1.22} \\
% \midrule
 Average & { 3.60} {\scriptsize$\pm$ 5.29} \\
 Minmax & 35.65 {\scriptsize$\pm$ 11.47} \\
 Oracle & { 52.21} {\scriptsize$\pm$ 4.31} \\
% \midrule
% Oracle DRO & Oracle& \underline{ 57.49} {\scriptsize$\pm$ 3.98} \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:biased_sst_95_model_selection} Effect of model selection criterion on robust validation accuracy.}
\end{table}

